MIRAGE: Multimodal Immersive Reasoning and Guided Exploration for Red-Team Jailbreak Attacks

While safety mechanisms have significantly progressed in filtering harmful text inputs, MLLMs remain vulnerable to multimodal jailbreaks that exploit their cross-modal reasoning capabilities. We present MIRAGE, a novel multimodal jailbreak framework that exploits narrative-driven context and role immersion to circumvent safety mechanisms in Multimodal Large Language Models (MLLMs). By systematically decomposing the toxic query into environment, role, and action triplets, MIRAGE constructs a multi-turn visual storytelling sequence of images and text using Stable Diffusion, guiding the target model through an engaging detective narrative. This process progressively lowers the model's defences and subtly guides its reasoning through structured contextual cues, ultimately eliciting harmful responses. In extensive experiments on the selected datasets with six mainstream MLLMs, MIRAGE achieves state-of-the-art performance, improving attack success rates by up to 17.5% over the best baselines. Moreover, we demonstrate that role immersion and structured semantic reconstruction can activate inherent model biases, facilitating the model's spontaneous violation of ethical safeguards. These results highlight critical weaknesses in current multimodal safety mechanisms and underscore the urgent need for more robust defences against cross-modal threats.

==> sec/7_future_work.tex <==
\section{Future Work}
Future research on MIRAGE can extend beyond static visual and textual inputs to explore more sophisticated multimodal attack strategies. One promising direction is the integration of dynamic sequences, such as video inputs and audio-based interactions, which could enhance attack stealthiness and increase success rates. By leveraging sequential multimodal data, attackers may be able to bypass safety mechanisms more effectively, as current defence strategies are primarily optimized for static inputs. 

To mitigate the risks posed by MIRAGE, defence strategies should incorporate dynamic safety validation mechanisms during inference. One potential approach is Multi-Turn Safety Validation, which detects cross-turn textual evolution and identifies instances where the model’s responses gradually approach sensitive or unsafe outputs, enabling early intervention and mitigation. Furthermore, Multimodal Fusion Anomaly Detection could be employed, utilizing Self-Supervised Learning (SSL) to learn patterns across image, text, and user interaction behaviours. By analyzing deviations from normal user interaction distributions, this method could identify and prevent potential MIRAGE attacks before they successfully manipulate the model.
